Shape-Aware Monocular 3D Object Detection

The detection of 3D objects through a single perspective camera is a challenging issue. The anchor-free and keypoint-based models receive increasing attention recently due to their effectiveness and simplicity. However, most of these methods are vulnerable to occluded and truncated objects. In this paper, a single-stage monocular 3D object detection model is proposed. An instance-segmentation head is integrated into the model training, which allows the model to be aware of the visible shape of a target object. The detection largely avoids interference from irrelevant regions surrounding the target objects. In addition, we also reveal that the popular IoU-based evaluation metrics, which were originally designed for evaluating stereo or LiDAR-based detection methods, are insensitive to the improvement of monocular 3D object detection algorithms. A novel evaluation metric, namely average depth similarity (ADS) is proposed for the monocular 3D object detection models. Our method outperforms the baseline on both the popular and the proposed evaluation metrics while maintaining real-time efficiency.

==> experiments1.tex <==
\section{Experiments}
\label{sec:experiments}
\begin{table*}[h!]
  \caption{Ablation study on the KITTI \textbf{val} sets for cars.}
  \label{tab:ablations}
  \resizebox{\textwidth}{!}{%
      \begin{tabular}{l|lll|lll|lll}
      \toprule
      \multirow{2}{*}{Approaches}     & \multicolumn{3}{c|}{$\text{AP}_{3D}$}                                                                             & \multicolumn{3}{c|}{$\text{AP}_{2D}$}                                                                            & \multicolumn{3}{c}{ADS}                                                                 \\
                                      & Easy                           & Moderate                  & Hard                              & Easy                              & Moderate                          & Hard                              & Easy                            & Moderate                        & Hard                           \\
      \midrule
      \color{red}MonoFlex*                       & 21.74                           & 15.79                            & 13.32                           & 96.56                           & 90.52                           & 80.89                           & 69.59                           & 60.16                           & 53.02                           \\
      \color{red}+ Center Sampling               & 23.25                           & 16.78                            & 14.81                           & 96.77                           & 90.81                           & 83.49                           & 70.00                           & 60.79                           & 54.96                           \\
      \color{red}+ Center Sampling + Shape-Aware & 24.92                           & 18.39                            & 15.56                           & 99.09                           & 91.13                           & 83.72                           & 73.53                           & 62.68                           & 56.61                           \\
      \bottomrule
      \end{tabular}
  }
\end{table*}


\begin{table*}[ht!]
  \centering
  \caption{
    Comparisons on the KITTI benchmark. 
    For models marked with *, we evaluate their performance 
    on the \textit{val} set by training with official codes. 
    For other models, their results on the \textit{val} set are 
     either cited from their papers or by evaluating the released pretrained model from the authors.
    Methods are ordered by their ${\text{AP}_{3D}}$ values under the moderate setting.
    For clarity, the best results are in {\color{red}red}, while the second is highlighted in {\color{blue}blue}. 
  }
    \begin{tabular}{l|c|lll|lll}
    \toprule
    \multicolumn{1}{c|}{\multirow{2}[0]{*}{Name}} & \multirow{2}[0]{*}{Extra Dataset} & \multicolumn{3}{c|}{$\text{AP}_{3D}$ (test/val)}                                                                          & \multicolumn{3}{c}{${\text{ADS}}$ (val)} \\
                                                  &                                   & Easy                                   & \textbf{Moderate}                      & Hard                                    & Easy                & \textbf{Moderate}        & Hard \\
    \midrule
    AutoShape \cite{liu2021autoshape}             & KINS                              & 22.47/20.09                            & 14.17/14.65                            & 11.36/12.07                             & -                   & -                        & -  \\
    LPCG-M3D-RPN \cite{peng2021lidar}             & KITTI raw                         & 22.73/26.17                            & 14.82/19.61                            & 12.88/16.80                             & -                   & -                        & -  \\
    DD3D \cite{park2021pseudo}                    & DDAD15M                           & 23.22/ -                               & 16.34/ -                               & 14.20/ -                                & -                   & -                        & -  \\
    LPCG-MonoFlex \cite{peng2021lidar}            & KITTI raw                         & 25.56/31.15                            & 17.80/23.42                            & 15.38/20.60                             & -                   & -                        & -  \\
    \hline
    MonoRUn \cite{chen2021monorun}                & \multirow{7}[0]{*}{None}          & 19.65/21.63                            & 12.30/15.22                            & 10.58/12.83                             & 67.95               & 58.91                    & 52.94  \\
    Ground-Aware* \cite{liu2021ground}            &                                   & 21.65/23.14                            & 13.25/15.71                            & 9.91/11.76                              & 69.42               & 54.47                    & 42.51  \\
    MonoFlex \cite{zhang2021objects}              &                                   & 19.94/24.22                            & 13.89/17.34                            & 12.07/15.14                             & 71.59               & {\color{blue}62.19}      & {\color{blue}56.10}\\
    DLE* \cite{liu2021deep}                       &                                   & {\color{red}24.23}/{\color{blue}25.58} & 14.33/16.50                            & 10.30/12.27                             & 70.26               & 56.44                    & 43.01  \\
    GUPNet \cite{lu2021geometry}                  &                                   & 22.26/23.19                            & 15.02/16.23                            & 13.12/13.57                             & 71.17               & 59.32                    & 52.14  \\
    MonoCon \cite{liu2022monocon}                &                                   & 22.50/{\color{red}26.33}               & {\color{blue}16.46}/{\color{red}19.03} & {\color{red}13.95}/{\color{red}16.00}   & {\color{blue}72.15} & 60.29                    & 54.40  \\
    Ours                                          &                                   & {\color{blue}23.84}/24.92              & {\color{red}16.52}/{\color{blue}18.39} & {\color{blue}13.88}/{\color{blue}15.56} & {\color{red}73.53}  & {\color{red}62.68}       & {\color{red}56.61}  \\
    \bottomrule
    \end{tabular}%
  \label{tab:performance}%
\end{table*}%


%\begin{table*}[h!]
%  \centering
%  \caption{The effect of result sampling.}
%  \label{tab:result_sampling}
%  % \resizebox{\textwidth}{!}{%
%      \begin{tabular}{l|lll|lll|lll}
%      \toprule
%                               & \multicolumn{3}{c|}{$\text{AP}_{2D}$}               & \multicolumn{3}{c|}{${\text{AP}_{3D}}$} & \multicolumn{3}{c}{ADS}                                                                    \\
%      \multirow{-2}{*}{\color{blue}Approaches} & Easy           & Moderate        & Hard             & Easy      & Moderate & Hard     & Easy   & Moderate & Hard   \\
%      \midrule
%      Ours                     & 99.09          & 91.13           & 83.72            & 24.92     & 18.39    & 15.56    & 73.53  & 62.68    & 56.61  \\
%      Ours + Result Sampling   & 92.66          & 73.83           & 66.68            & 27.86     & 22.31    & 19.42    & 69.22  & 52.29    & 46.45           \\
%      \bottomrule
%      \end{tabular}
%  % }
%\end{table*}

Our method is evaluated on the popular KITTI dataset~\cite{Geiger2013IJRR, Geiger2012CVPR} in comparison to state-of-the-art methods. The dataset consists of \textit{7,481} training images and \textit{7,518} testing images. Since only two evaluations per month on the \textit{test} set are allowed in the official website of KITTI, the training images are split into \textit{train} (3,712) and \textit{val} (3,769) sets following \cite{chen20153d}. All our models jointly predict three categories, including car, pedestrain, and cyclist.


The methods we consider in the experiment include one-stage center-based methods such as AutoShape~\cite{liu2021autoshape}, LPCG-MonoFlex~\cite{peng2021lidar}, MonoCon~\cite{liu2022monocon}, MonoFlex~\cite{zhang2021objects} and GUPNet~\cite{kendall2019geometry}. The comparison also covers one-stage anchor-based methods such as Ground-Aware~\cite{liu2021ground}, DLE~\cite{liu2021deep}, and LPCG-M3D-RPN~\cite{peng2021lidar} and one-stage FCOS-like method DD3D~\cite{park2021pseudo}. A two-stage method MonoRUn~\cite{chen2021monorun} is incorporated in our comparative study as well. In the evaluation, MonoFlex~\cite{zhang2021objects} that is retrained with the same settings as our method is treated as the comparison baseline. For clarity, this run is given as ``MonoFlex*'', while the run that is loyal to the original paper is given as ``MonoFlex''.


\subsection{Ablation Study}\label{sec:ablation}
%\begin{table}[htbp]
%  \centering
%  \caption{Improvements on other categories. Methods are evaluated using the ${\text{AP}_{3D}}$ metric on the KITTI \textit{val} set.}
%    \begin{tabular}{l|rrr|rrr}
%    \toprule
%    \multirow{2}[0]{*}{Approaches} & \multicolumn{3}{c|}{Pedestrain} & \multicolumn{3}{c}{Cyclist} \\
%                                   & Easy & Mod. & Hard              & Easy  & Mod.  & Hard  \\
%    \midrule
%    Baseline                       & 5.47 & 4.40 & 3.47              & 5.24  & 2.69  & 2.59  \\
%    Ours                           & 8.80 & 6.88 & 5.78              & 6.77  & 3.24  & 3.12  \\
%    \bottomrule
%    \end{tabular}%
%  \label{tab:ped_cyc_apthree}%
%\end{table}%
%
%% Table generated by Excel2LaTeX from sheet 'ads val ped cyc.'
%\begin{table}[htbp]
%  \centering
%  \caption{Improvements on other categories. Methods are evaluated using the ${\text{ADS}}$ metric on the KITTI \textit{val} set.}
%    \begin{tabular}{l|rrr|rrr}
%    \toprule
%    \multirow{2}[0]{*}{Approaches} & \multicolumn{3}{c|}{Pedestrain} & \multicolumn{3}{c}{Cyclist} \\
%                                   & Easy & Mod.  & Hard             & \multicolumn{1}{l}{Easy} & \multicolumn{1}{l}{Mod.} & \multicolumn{1}{l}{Hard} \\
%    \midrule
%    Baseline & 46.23  & 36.84  & 31.12  & 36.41  & 21.28  & 19.94  \\
%    Ours     & 53.34  & 44.56  & 37.13  & 44.18  & 26.86  & 24.93  \\
%    \bottomrule
%    \end{tabular}%
%  \label{tab:ped_cyc_ads}%
%\end{table}%
In our first experiment, an ablation study is conducted to show the contributions from center sampling (CS) and shape-aware training (SA), that are introduced by us. We observed that, when solely applying center sampling, we can improve ${\text{AP}_{3D}}$ and ${\text{ADS}}$ 
by {\color{blue}6.27\% and 1.05\%} respectively on the moderate objects. When the shape-aware
auxiliary training head is further integrated, extra 9.59\% and 3.11\% improvement in the ${\text{AP}_{3D}}$ and ${\text{ADS}}$ metrics are observed. This improvement is consistent on the pedestrain and cyclist categories, as shown in Table \ref{tab:ped_cyc_apthree} and Table \ref{tab:ped_cyc_ads}.

%In Table \ref{tab:result_sampling}, we evaluate the result sampling strategy with 
%several evaluation metrics. For result sampling, objects with depth 
%larger than $t_z = 20$ is copied and pasted at 
%$$z' \in \left\{z + \Delta z ~\big|~ \Delta z \in \left\{-2, -1, -0.5, 0, 0.5, 1, 2\right\}\right\},$$ 
%the hyper-parameter $\lambda$ is set to 80. For generated 3D boxes, their corresponding 
%2D boxes are updated with the projection of the 3D ones. It can be 
%observed from Table \ref{tab:result_sampling} that, while result sampling 
%can significantly improve the ${\text{AP}_{3D}}$, the improvement is achieved with 
%sacrificing of ${\text{AP}_{2D}}$ and ${\text{ADS}}$. While result sampling can achieve 
%a better trade-off between precision and recall when evaluating ${\text{AP}_{3D}}$, 
%it makes no contribution to the quality of 2D bounding boxes. Therefore, 
%it's not surprising that it produces a lower ${\text{AP}_{2D}}$. The calculating of ${\text{ADS}}$ is 
%based on the matching of 2D bounding boxes, therefore it's {\color{red}cannot} be cheated 
%by tricks like result sampling. As shown in Table \ref{tab:result_sampling}, 
%${\text{ADS}}$ goes down when result sampling is applied. In our experiments, we evaluate 
%the performance of models with ${\text{ADS}}$ to enable a comprehensive understanding 
%of the model performance. 

%\begin{figure}[h]
%  \centering
%  \subcaptionbox{}{
%    \centering
%    \includegraphics[height=3.9cm]{figures/ap_and_ads/ap3d_and_ads.pdf}
%  }
%  \subcaptionbox{}{
%    \centering
%    \includegraphics[height=3.9cm]{figures/ap_and_ads/ap2d_and_ads.pdf}
%  }
%  \caption{
%    ${\text{ADS}}$ vs ${\text{AP}_{3D}}$ and ${\text{AP}_{2D}}$ on the KITTI val set.
%    \label{fig:ap_and_ads}
%  }
%\end{figure}

\begin{table}[h!]
  \centering
  \caption{Comparison between different RoI feature extractors. Experiments are conducted on the KITTI \textit{val} set}
  \label{tab:roi_feature_extractors}
  % \resizebox{\textwidth}{!}{%
      \begin{tabular}{l|rrr|rrr}
      \toprule
                                               & \multicolumn{3}{c|}{${\text{AP}_{3D}}$} & \multicolumn{3}{c}{${\text{ADS}}$}                                                                    \\
      \multirow{-2}{*}{Methods} & \multicolumn{1}{c}{Easy} & Mod.      & Hard  & Easy   & Mod. & Hard    \\
      \midrule
      MonoFlex*                    & 21.74       & 15.79     & 13.32 & 69.59   & 60.16    & 53.02  \\
      + RoIAlign                   & 19.97       & 14.65	   & 12.91 & 69.19	 & 59.79	  & 52.86  \\
      + Ours                       & 24.92       & 18.39     & 15.56 & 73.53   & 62.68    & 56.61  \\
      \bottomrule
      \end{tabular}
  % }
\end{table}

In our second experiment, we confirm the choice of feature expanding instead of RoIAlignment in the pipeline of segmentation head. As shown in  Table~\ref{tab:roi_feature_extractors}, the performance of the detector drops when RoIAlignment used as the feature extractor in the segmentation head. In contrast, considerable improvement is observed when the RoIAlignment is replaced by feature expanding (shown in Figure~\ref{fig:feature_expanding}) in the feature extractor. As discussed earlier, the misalignment between the RoI-based and center-based representation leads to potential conflicts between two training heads.

\subsection{Performance Analysis}
In this section, the performance of method is studied on both the \textit{test} and \textit{val} set of 
the KITTI benchmark in comparison to state-of-the-art methods. The 3D average precision ${\text{AP}_{3D}}$ and the 
average depth similarity ${\text{ADS}}$ are used for evaluation. Note that we only 
evaluate ${\text{ADS}}$ on the \textit{val} set since the ground-truth of 
the \textit{test} set is not available. Evaluation metrics are  
divided into easy, moderate, and hard settings according to the height, 
occlusion, and truncation level of objects. All evaluation metrics use 
40 recall points instead of 11 recall points as recommended in 
\cite{simonelli2019disentangling}. 
We report the evaluation result on the KITTI \textit{test} set in 
Table~\ref{tab:performance}. From the table, we can observe that our 
method achieved competitive performance with the current SOTA, and 
outperforms it on the ${\text{AP}_{3D}}$ metric on the moderate setting. 
Qualitative results are illustrated in Figure~\ref{fig:qualitative_results}.

For intuitive understanding, we compare the ${\text{AP}_{3D}}$ and ${\text{ADS}}$ metric of 
many models on a 2D coordinate system, as illustrated in 
Fig~\ref{fig:ap_and_ads} (a).
From this figure, we can see that models with higher ${\text{AP}_{3D}}$ do not 
necessarily produce higher ${\text{ADS}}$. Our method is competitive when using either the 
${\text{AP}_{3D}}$ or the ${\text{ADS}}$ metric.
In our opinion, neither of 
${\text{AP}_{3D}}$ and ${\text{ADS}}$ is perfect, 
they both have artifacts. The former one can be easily fooled by 
precision-recall trade-off tricks as discussed in Section \ref{sec:ablation}. 
The latter one can only evaluate the depth similarity, leaving 3D 
pose and dimension predictions ignored. 
During the development of our model, we encourage our model to produce 
higher ${\text{AP}_{3D}}$ and ${\text{ADS}}$ at the same time. 

Similarly, we can observe the relationship between 
${\text{AP}_{2D}}$ and ${\text{ADS}}$ from Figure~\ref{fig:ap_and_ads} (b).
Since the computation of ${\text{ADS}}$ is based on the matching of 2D bounding boxes, 
it's reasonable to see a trend that methods with higher ${\text{AP}_{2D}}$ tend to produce higher ${\text{ADS}}$. 
However, the ${\text{ADS}}$ is not totally decided by the ${\text{AP}_{2D}}$. For 
example, although MonoFlex and MonoDLE have higher ${\text{AP}_{2D}}$, they 
are inferior in ${\text{ADS}}$ when compared with our model.

\begin{figure*}
  \centering
  \includegraphics[align=c,width=6.3cm]{figures/qualitative_results_valset/fig-valset-135-det-proj.pdf}
  \includegraphics[align=c,width=6.3cm]{figures/qualitative_results_valset/fig-valset-135-seg.pdf}
  \raisebox{-0.18\height}{\includegraphics[align=c,width=5.0cm]{figures/qualitative_results_valset/fig-valset-135-det-bev.pdf}}

  \includegraphics[align=c,width=6.3cm]{figures/qualitative_results_valset/fig-valset-1125-det-proj.pdf}
  \includegraphics[align=c,width=6.3cm]{figures/qualitative_results_valset/fig-valset-1125-seg.pdf}
  \raisebox{-0.18\height}{\includegraphics[align=c,width=5.0cm]{figures/qualitative_results_valset/fig-valset-1125-det-bev.pdf}}

  \includegraphics[align=c,width=6.3cm]{figures/qualitative_results_valset/fig-valset-404-det-proj.pdf}
  \includegraphics[align=c,width=6.3cm]{figures/qualitative_results_valset/fig-valset-404-seg.pdf}
  \raisebox{-0.18\height}{\includegraphics[align=c,width=5.0cm]{figures/qualitative_results_valset/fig-valset-404-det-bev.pdf}}

  \includegraphics[align=c,width=6.3cm]{figures/qualitative_results_valset/fig-valset-408-det-proj.pdf}
  \includegraphics[align=c,width=6.3cm]{figures/qualitative_results_valset/fig-valset-408-seg.pdf}
  \raisebox{-0.18\height}{\includegraphics[align=c,width=5.0cm]{figures/qualitative_results_valset/fig-valset-408-det-bev.pdf}}
  
  \caption{Qualitative results on the KITTI \textit{val} set. \label{fig:qualitative_results}}
\end{figure*}

{\color{blue}
\subsection{Analysis on Occluded Objects}
% Table generated by Excel2LaTeX from sheet 'Occlusion Analysis'
\begin{table}[htbp]
  \centering
  \caption{
    \color{blue}
    Comparison between occluded and fully visible objects. We compare the 
    ${\text{AP}_{3D}}$ and ${\text{ADS}}$ for cars on the KITTI \textit{val} set. 
  }
    \begin{tabular}{l|rr|rr}
    \toprule
    \multicolumn{1}{c|}{\multirow{2}[0]{*}{Approaches}} & \multicolumn{2}{c|}{${\text{AP}_{3D}}$}                           & \multicolumn{2}{c}{${\text{ADS}}$} \\
                                                        & \multicolumn{1}{c}{Fully Visible} & \multicolumn{1}{c|}{Occluded} & \multicolumn{1}{c}{Fully Visible} & \multicolumn{1}{c}{Occluded} \\
    \midrule
    MonoFlex* & 13.34 & 6.29 & 62.35 & 43.59 \\
    Ours     & 15.21 & 8.92 & 64.68 & 50.55 \\
    \bottomrule
    \end{tabular}%
  \label{tab:occlusion_analysis}%
\end{table}%
The KITTI dataset provides each ground-truth label with an occlusion state 
and a truncation score. There are four kinds of occlusion states: 
$o \in \left\{0, 1, 2, 3\right\}$, where 0, 1, 2, and 3 means 
fully visible, partly occluded, largely occluded, and unknown respectively. 
The truncation score $t$, which refers 
to the object leaving the image boundaries, is a float value that 
ranges from 0 to 1.

To investigate the performance of our method on occluded objects, 
in this subsection, we divide objects into two categories, fully visible and occluded, 
according to their occlusion state and truncation score. 
Note that truncated objects are also considered as occluded ones here for 
convenience since the truncation also reduces the visible area of 
the object. 
Objects with 
occlusion state and truncation score equal to 0 are marked as 
fully visible. Others with occlusion states equal to 1 or 2, 
or truncation scores larger than \textit{0} are marked as occluded. 
If an object can neither be categorized as fully visible nor occluded 
since its 
occlusion state is 3 (unknown), it's ignored in the evaluation, i.e., 
we do not count these objects as false positives when they are detected.
Objects with a height smaller than 25px are also ignored as in the 
moderate setting of the original KITTI benchmark.

The evaluation results are reported in Table \ref{tab:occlusion_analysis}. 
As indicated by the data, it's easy to see that occluded objects are more difficult 
to be accurately located in the 3D space. It can be observed that our 
method significantly improves the ${\text{AP}_{3D}}$ and the ${\text{ADS}}$ 
for occluded objects by 41.81\% and 15.97\%. Meanwhile, the performance on 
fully visible objects can also be benefited from our method. The 
${\text{AP}_{3D}}$ and the ${\text{ADS}}$ for fully visible objects are 
improved by 14.02\% and 3.74\% respectively.
}


==> preliminary.tex <==
\section{Preliminary}
\label{sec:preliminary}


We built our baseline model basically upon the MonoFlex \cite{zhang2021objects}
network, which takes only one RGB image as the input and generates 2D 
object bounding boxes with 3D attributes for each object. Then through 
post-processing, the 3D pose can be decoded from the predicted attributes. 

The task assumes that the intrinsic parameters are known. The intrinsic parameters of a 
camera can be organized as a $3\times 3$ matrix:
$$
\left(
  \begin{matrix}
    f & 0 & c_u \\
    0 & f & c_v \\
    0 & 0 & 1
  \end{matrix}
\right),
$$
{\color{red}where f is the focal length. $(c_u, c_v)$ is the principle point of the image.}


\begin{figure}
  \centering\includegraphics[width=0.8\linewidth]{figures/representative_center/representative_center.pdf}
  \caption{The representative centers of non-truncated and truncated objects.
  \label{fig:representative_center}}
\end{figure}

\subsection{\color{red}Decoupling of Inside/Truncated Objects}
In Center-based detectors \cite{zhou2019objects,zhang2021objects}, each object is represented with a representative center {\color{red}$\mathbf x_r$}. As 
illustrated in Figure~\ref{fig:representative_center}, 
MonoFlex takes the 2D projection of the 3D bounding box center 
$\mathbf x_c$ as the representative center, and generate the ground-truth heatmap with Gaussian kernel like \cite{li2020rtm3d}. If $\mathbf x_c$ is out of image, then the intersection point $\mathbf x_I$ of the line 
$(\mathbf x_b, \mathbf x_c)$ and the image edge is used as the 
representative center, where $\mathbf x_b$ is the center of the 2D 
bounding box. Also, for outside objects, $\mathbf x_I$ is predicted with the edge heatmap\cite{zhang2021objects}, which is essentially a 1D Gaussian. 
{\color{red}
In addition, the edge fusion module is used to decouple 
the learning of truncated objects by applying 1D 
convolution on edge features extracted from four 
boundaries of the input image.
}

\subsection{Object Detection} 
{\color{blue}
To offer a general view, we list all attributes to be regressed in Table \ref{tab:heads_and_parameters}.
Then, we introduce how to make use of them in this subsection.
}

\begin{table}
  \centering
  \caption{\color{blue}Object attributes to be regressed.}
    \begin{tabular}{l|r}
    \toprule
    \multirow{1}[0]{*}{Name} & \multicolumn{1}{c}{Channels} \\
    \midrule
    Depth                    & 1  \\
    Orientation              & 16 \\
    2D Bounding Box          & 4  \\
    3D Dimensions            & 3  \\ 
    Center Offset            & 2  \\ 
    Keypoints                & 20 \\
    Uncertainties            & 4  \\
    \bottomrule
    \end{tabular}%
  \label{tab:heads_and_parameters}%
\end{table}

\textbf{2D Detection.} 
{\color{blue}
Boxes are represented as distances 
from the representative center to four sides of the 2D bounding box following FCOS \cite{tian2019fcos}. 
GIoU loss \cite{Rezatofighi_2019_CVPR} is adopted for learning 2D bounding 
boxes since it is robust to object scale changes.
}

\textbf{3D Detection.}
As illustrated in Figure~\ref{fig:keypoint_definition}, the 
head predicts 10 keypoints for each object, from which we 
can extract five vertical lines. 
Then, with known camera intrinsic parameters, the depth 
value of vertical line $l$ is estimated by utilizing the relative proportion 
between pixel height and estimated 
object height \cite{zhang2021objects,cai2020monocular}:
$$z_l=\frac{f\times h}{h_l}$$
where  $f$ is the focal length. $h_l$ and $h$ are the height of line $l$ in pixel 
and the 3D height of the object respectively. Five vertical lines are 
divided into 
three groups, and the depth value of each vertical line 
is averaged within each group, resulting in three independent 
center depth values.
In addition, the model also directly regresses a 
depth value, so there are 4 depth values in total for each 
object. 
%\begin{figure}
%  \centering
%  \includegraphics[width=0.6\linewidth]{figures/keypoint_definition/keypoint_definition2.pdf}
%  \caption{
%    Five vertical lines can be extracted from 10 keypoints. These 
%    lines are divided into three groups, each of which can produce an 
%    independent depth prediction. \label{fig:keypoint_definition}
%  }
%\end{figure}

The final depth is obtained by computing uncertainty-weighted 
average:
$$
z_{final} = \left(\sum_{i=1}^{4}\frac{z_i}{\sigma_i}\right)/\left(\sum_{i=1}^{4}\frac{1}{\sigma_i}\right)
$$
where the uncertainty estimation branch is trained under 
the laplacian uncertainty loss
\cite{kendall2019geometry,chen2021monorun,kendall2017uncertainties,kendall2018multi}.

With predicted projected 3D center 
$\mathbf x_c = (u_c, v_c)$, The object location can be decoded as:
$$
(x, y, z) = \left(\frac{(u_c - c_u)z}{f}, \frac{(v_c - c_v)z}{f}, z\right)
$$
where $(c_u, c_v)$ is the principle point. 

For dimension estimation, the relative changes with 
respect to the average dimension is predicted. For each 
class $c$, the average dimension is denoted as 
$(\bar h_c, \bar w_c, \bar l_c)$, the L1 loss for dimension 
regress is defined as: 
$$
L_{dim} = \sum_{k\in{h, w, l}} \left| \bar k_c e^{\delta_k} - k^* \right|
$$
where $k*$ is the ground-truth dimension.

MultiBin loss \cite{mousavian20173d} is used to estimate the local 
orientation $\alpha$. The global 
orientation $r_y$ can be obtained by calculating:
$$
r_y = \alpha + \arctan(x/z).
$$

The final 3D bounding box is then encoded as $(x, y, z, w, h, l, r_y)$. 
We refer readers to \cite{zhang2021objects} for more details of the 3D 
detection head.

{\color{red}
The Monocular 3D detection pipeline proposed by MonoFlex 
decouples the learning and prediction of 
inside/truncated objects, and formulates the object 
detection tasks as an uncertainty-weighted ensemble of 
multiple approaches, leading to more robust and accurate 
detection. 
However, while similar to truncation, the 
occlusion problem is few investigated in prior papers 
and still remains unresolved. The learning of 
partially visible objects, including truncated and 
occluded ones, is easy to fall into over fitting. In 
this paper, we propose 
to improve the generalization ability of the monocular 
detection model by learning shape-aware features. We will 
detail our method in the subsequent section.
}
